Chart-to-Experience: Benchmarking Multimodal LLMs for Predicting Experiential Impact of Charts

The field of Multimodal Large Language Models (MLLMs) has made remarkable progress in visual understanding tasks, presenting a vast opportunity to predict the perceptual and emotional impact of charts. However, it also raises concerns, as many applications of LLMs are based on overgeneralized assumptions from a few examples, lacking sufficient validation of their performance and effectiveness. We introduce Chart-to-Experience, a benchmark dataset comprising 36 charts, evaluated by crowdsourced workers for their impact on seven experiential factors. Using the dataset as ground truth, we evaluated capabilities of state-of-the-art MLLMs on two tasks: direct prediction and pairwise comparison of charts. Our findings imply that MLLMs are not as sensitive as human evaluators when assessing individual charts, but are accurate and reliable in pairwise comparisons.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> src/tables/RWs.tex <==
\begin{table}[h!]
\caption{Three closely related domains.}
\small
\setlength{\tabcolsep}{0.6em}
\renewcommand{\arraystretch}{1.0}
\centering{
\scalebox{0.92}{
\begin{tabu}{l|cccc|}
\toprule
\textbf{Domain} & \textbf{\shortstack{Paper1}} & \textbf{Paper2} & \textbf{\shortstack{Paper3}} & \textbf{Ours} \\ \hline
Emotion Prediction for Images using MLLMs &  &  &  & - \\ 
Chart Understanding using MLLMs &  &  &  & - \\ 
Evaluating MLLM as-a-Judge &  &  &  & - \\ 
\bottomrule
\end{tabu} %
}}
\label{table:descriptive of each factor}
\vspace{-8pt}
\end{table}

% can colored to resemble heatmap
% or to distinguish Models and Human data?
% 

% % Llama 3.2 = Llama 3.2 11B Vision Instruct
% HousePrice	    5.49	0.67	3.97	0.64	2.94	0.68	5.36	0.68	4.85	0.79	4.94	0.75
% COVID	        5.41	0.94	4.06	0.59	2.99	0.73	5.06	1.22	5.19	0.83	5.16	0.87
% GlobalWarming	5.76	0.51	4.04	0.48	2.91	0.60	5.41	0.78	4.82	0.85	5.11	0.75

% Claude Sonnet 3.5 v1
% HP	5.63	0.91	6.23	0.74	6.16	0.65	4.58	0.89	5.51	0.91	5.62	0.85	5.04	0.82
% COVID	5.65	0.79	6.19	0.74	6.31	0.56	4.87	0.73	5.46	0.76	5.57	0.79	5.30	0.83
% GW	5.93	0.81	6.50	0.62	6.51	0.57	5.28	0.89	5.70	0.77	5.93	0.79	5.20	0.74





% \begin{table*}[h!]
% \caption{Means~(M) and standard deviations~(SD) for each topic and factor.}
% \small
% \setlength{\tabcolsep}{0.6em}
% \renewcommand{\arraystretch}{1.1}
% \centering{
% \begin{tabu}{ll|cc|cc|cc|cc|cc|cc|cc|}
% % \begin{tabu}{lc:cc:cc:cc:cc:cc:cc:c}
% % \hline
% \toprule
% \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Memorability}} & \multicolumn{2}{c|}{\textbf{Interest}} & \multicolumn{2}{c|}{\textbf{Trustworthiness}} & \multicolumn{2}{c|}{\textbf{Empathy}} & \multicolumn{2}{c|}{\textbf{\shortstack{Aesthetic\\Pleasure}}} & \multicolumn{2}{c|}{\textbf{Intuitiveness}} & \multicolumn{2}{c|}{\textbf{Comfort}} \\
% % \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Mem.}} & \multicolumn{2}{c|}{\textbf{Int.}} & \multicolumn{2}{c|}{\textbf{Tru.}} & \multicolumn{2}{c|}{\textbf{Emp.}} & \multicolumn{2}{c|}{\textbf{Aes.}} & \multicolumn{2}{c|}{\textbf{Itt.}} & \multicolumn{2}{c|}{\textbf{Cft.}} \\
% Topic & Evaluator & M(SD) & \tau(p) & M(SD) & \tau(p) & M(SD) & \tau(p) & M(SD) & \tau(p) & M(SD) & \tau(p) & M(SD) & \tau(p) & M(SD) & \tau(p)\\ \hline
% \multirow{4}{*}{\shortstack{House\\Prices}} & Human & 4.40(2.20) & - & 5.24(1.65) & - & 5.18(1.74) & - & 4.43(1.82) & - & 4.78(1.98) & - & 4.81(1.89) & - & 4.89(1.86) & - \\
%  & Sonnet-3.5 & 5.88(0.80) & - & 6.40(0.66) & - & 6.27(0.59) & - & 4.78(0.75) & - & 5.59(0.87) & - & 5.83(0.78) & - & 5.34(0.74) & - \\
%  & GPT-4o & 5.32(0.78) & - & 5.39(0.77) & - & 5.79(0.75) & - & 4.11(0.87) & - & 5.08(0.72) & - & 5.32(0.74) & - & 5.07(0.67) & - 
%  \\
%  & Llama 3.2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  \hline
% \multirow{4}{*}{COVID} & Human & 4.03(2.14) & - & 5.22(1.63) & - & 5.10(1.71) & - & 4.49(1.82) & - & 4.91(1.76) & - & 4.62(1.74) & - & 4.95(1.79) & - \\
% & Sonnet-3.5 & 5.76(0.81) & - & 6.33(0.72) & - & 6.52(0.55) & - & 4.96(0.77) & - & 5.50(0.77) & - & 5.74(0.82) & - & 5.59(0.79) & - \\
% & GPT-4o & 5.23(0.74) & - & 5.18(0.81) & - & 5.98(0.71) & - & 4.55(0.82) & - & 5.02(0.67) & - & 5.29(0.68) & - & 5.22(0.65) & - 
% \\
% & Llama 3.2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% \hline
% \multirow{4}{*}{\shortstack{Global\\Warming}} & Human & 4.40(2.20) & - & 5.49(1.66) & - & 4.99(1.78) & - & 4.53(1.76) & - & 5.00(1.90) & - & 4.83(1.93) & - & 4.83(1.97) & - \\
% & Sonnet-3.5 & 6.01(0.79) & - & 6.49(0.62) & - & 6.57(0.57) & - & 5.28(0.81) & - & 5.68(0.81) & - & 5.93(0.82) & - & 5.29(0.82) & - \\
% & GPT-4o & 5.34(0.59) & - & 5.73(0.69) & - & 6.05(0.66) & - & 4.68(0.69) & - & 5.36(0.68) & - & 5.55(0.64) & - & 5.40(0.59) & - 
% \\
% & Llama 3.2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% % \hline
% \bottomrule
% \end{tabu} %
% }
% \label{table:descriptive of each factor}
% % \vspace{-22pt}
% \end{table*}
% % % Llama 3.2 = Llama 3.2 11B Vision Instruct
